Discovering Parametric Activation Functions

Recent studies have shown that the choice of activation function can significantly affect the performance of deep learning networks. However, the benefits of novel activation functions have been inconsistent and task dependent, and therefore the rectified linear unit (ReLU) is still the most commonly used. This paper proposes a technique for customizing activation functions automatically, resulting in reliable improvements in performance. Evolutionary search is used to discover the general form of the function, and gradient descent to optimize its parameters for different parts of the network and over the learning process. Experiments with four different neural network architectures on the CIFAR-10 and CIFAR-100 image classification datasets show that this approach is effective. It discovers both general activation functions and specialized functions for different architectures, consistently improving accuracy over ReLU and other activation functions by significant margins. The approach can therefore be used as an automated optimization step in applying deep learning to new tasks.

==> figures/changing_size.tex <==
\begin{figure*}
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \includegraphics[width=0.33\linewidth]{images/width.pdf}
    \includegraphics[width=0.33\linewidth]{images/depth.pdf}
    \includegraphics[width=0.33\linewidth]{images/resnetv2.pdf}
    \end{adjustbox}
    \caption{CIFAR-100 test accuracy for different neural networks and activation functions.  Accuracy with ReLU is shown in blue, and accuracy with the specialized activation functions in red.  The relative improvement of the specialized functions over ReLU is shown as a dotted green line, according to the axis values on the right of each plot.  \textbf{Left:} The depth of Wide ResNet is fixed at 10, and the width varies from 1 to 16.  \textbf{Center:} The depth of Wide ResNet varies from 10 to 34, while the width is fixed at four.  \textbf{Right:} The depth of Preactivation ResNet ranges from 20 to 164.  The width and depth of a network can affect how much a specialized activation function outperforms ReLU.}
    \label{fig:changing_size}
\end{figure*}



==> figures/moving_acc_runtime.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/moving_acc.pdf}
    % Maybe we don't need this one.  What's the point it is making anyway?
    % \includegraphics[width=0.49\linewidth]{images/moving_runtime.pdf}
    \caption{Average population fitness across time for two independent PANGAEA processes.  The plots show the average validation accuracy achieved with the $P=64$ most recently evaluated activation functions at any given time in the search process.  The two PANGAEA runs behave similarly, gradually discovering better activation functions as they explore the search space.}
    \label{fig:moving_acc_runtime}
\end{figure}

==> figures/repeated_results.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{ll}
        \toprule
        \textbf{Original PANGAEA Run}\\
        $\alpha x - \beta \log(\sigma(\gamma x))$ & 
        $71.01 {\scriptscriptstyle \pm 0.64}$ \\
        $\alpha x - \log(\sigma(\beta x))$ & 
        $70.30 {\scriptscriptstyle \pm 0.58}$ \\
        $\max\{\textrm{Swish}(x), 0\}$ & 
        $69.43 {\scriptscriptstyle \pm 0.69}$ \\
        \midrule
        
        \textbf{Additional PANGAEA Run 1} \\
        $\max \{ \min\{ \alpha \cdot x , \textrm{ELU}(x)\} , 0 \}$ & $70.53 {\scriptscriptstyle \pm 0.31}$\\ 
        $\alpha \cdot \max\left\{\beta \cdot \textrm{ReLU}\left(\frac{\textrm{Swish}(x)}{\gamma}\right), x\right\}$ & $70.52 {\scriptscriptstyle \pm 0.39}$\\
        $\max\{ \textrm{ReLU}(\textrm{Swish}(\alpha \cdot x)), \beta \cdot x\}$ & $70.44 {\scriptscriptstyle \pm 0.44}$\\
        \midrule
        
        \textbf{Additional PANGAEA Run 2} \\
        $\max\{ \textrm{Swish}(\alpha \cdot x), x \}$ & $\bm{71.03} {\scriptscriptstyle \pm 0.40}$\\
        $\max\{ \textrm{Swish}(x), \textrm{arcsinh}(\alpha \cdot \beta \cdot x)\}$ & $70.52 {\scriptscriptstyle \pm 0.35}$\\ 
        $\max\{ \textrm{Swish}(x), \textrm{arcsinh}(\alpha \cdot x)\}$ & $70.41 {\scriptscriptstyle \pm 0.38}$\\
        \midrule
        ReLU & $69.64 {\scriptscriptstyle \pm 0.65}$\\
        \bottomrule
    \end{tabular}
    \caption{Activation functions discovered with repeated independent PANGAEA runs on ResNet-v1-56.  Results shown are the CIFAR-100 test set accuracy aggregated over ten runs, shown as mean $\pm$ sample standard deviation.  Repeating PANGAEA from scratch produces activation functions that have different functional forms and yet achieve similarly high accuracy.}
    \label{tab:repeated_results}
\end{table}


==> figures/results_old.tex <==

\begin{table*}
    \centering
    \caption{CIFAR-100 test set accuracy shown as a median of ten runs, with mean $\pm$ sample standard deviation in parenthesis.  Asterisks indicate a statistically significant improvement in mean accuracy over ReLU, with * if $p \leq 0.05$, ** if $p \leq 0.01$, and *** if $p \leq 0.001$;  $p$-values are from one-tailed Welch's $t$-tests.  The top accuracy for each architecture is in bold, and results that are not statistically different from the top accuracy are also in bold.  Baseline activation function details are in \ref{ap:baseline}.\newline
    }
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{llll} \toprule
    & \textbf{WRN-10-4} & \textbf{ResNet-v1-56} & \textbf{ResNet-v2-56} \\ \midrule

    \textbf{Specialized for WRN-10-4}\\
    $\log(\sigma(\alpha x)) \cdot \textrm{arcsinh}(x)$ & 
    \cellcolor{black!5} \boldsymbol{$73.23$} {\scriptsize $(73.16 \pm 0.41)$ ***} &
    $11.15$ {\scriptsize $(19.34 \pm 20.14)$} &
    \boldsymbol{$72.05$} {\scriptsize $(64.30 \pm 21.32)$} \\
    
    $\log(\sigma(\alpha x)) \cdot \beta \textrm{arcsinh}(x)$ & 
    \cellcolor{black!5} \boldsymbol{$73.22$} {\scriptsize $(73.20 \pm 0.37)$ ***} &
    $05.78$ {\scriptsize $(18.63 \pm 21.04)$} &
    $55.40$ {\scriptsize $(45.88 \pm 30.70)$} \\
    
    $-\textrm{Swish}(\textrm{Swish}(\alpha x))$ & 
    \cellcolor{black!5} $72.38$ {\scriptsize $(72.49 \pm 0.55)$ ***} &
    $59.61$ {\scriptsize $(58.86 \pm 2.88)$} &
    $74.70$ {\scriptsize $(74.71 \pm 0.20)$ *} \\ 
    \midrule 

    \textbf{Specialized for ResNet-v1-56}\\
    $\alpha x - \beta \log(\sigma(\gamma x))$ & 
    $70.35$ {\scriptsize $(70.28 \pm 0.37)$} &
    \cellcolor{black!5} \boldsymbol{$70.82$} {\scriptsize $(71.01 \pm 0.64)$ ***} &
    $74.41$ {\scriptsize $(74.35 \pm 0.45)$} \\
    
    $\alpha x - \log(\sigma(\beta x))$ & 
    $70.62$ {\scriptsize $(70.47 \pm 0.53)$} &
    \cellcolor{black!5} $70.30$ {\scriptsize $(70.30 \pm 0.58)$ *} &
    $74.73$ {\scriptsize $(74.70 \pm 0.23)$ *} \\
    
    $\max\{\textrm{Swish}(x), 0\}$ & 
    $71.96$ {\scriptsize $(72.10 \pm 0.33)$ **} &
    \cellcolor{black!5} $69.46$ {\scriptsize $(69.43 \pm 0.69)$} &
    $74.97$ {\scriptsize $(74.97 \pm 0.25)$ **} \\
    \midrule 
    
    \textbf{Specialized for ResNet-v2-56}\\
    $\textrm{Softplus}(\textrm{ELU}(x))$ & 
    $71.51$ {\scriptsize $(71.36 \pm 0.34)$} &
    $69.94$ {\scriptsize $(69.96 \pm 0.39)$} &
    \cellcolor{black!5} \boldsymbol{$75.60$} {\scriptsize $(75.61 \pm 0.42)$ ***} \\
    
    $\min\{\log(\sigma(x)), \alpha \log(\sigma(\beta x))\}$ & 
    $72.05$ {\scriptsize $(72.04 \pm 0.34)$ **} &
    $69.63$ {\scriptsize $(69.56 \pm 0.48)$} &
    \cellcolor{black!5} $75.20$ {\scriptsize $(75.19 \pm 0.39)$ ***} \\
    
    $\textrm{SELU}(\textrm{Swish}(x))$ & 
    $01.00$ {\scriptsize $(01.00 \pm 0.00)$} &
    $01.00$ {\scriptsize $(01.00 \pm 0.00)$} &
    \cellcolor{black!5} $75.06$ {\scriptsize $(75.02 \pm 0.35)$ **} \\
    \midrule 
    
    \textbf{General Activation Functions}\\
    $\max\{\textrm{Swish}(x), \alpha \log (\sigma (\textrm{ReLU}(x)))\}$ & 
     $72.50$ {\scriptsize $(72.54 \pm 0.26)$ ***} &
     $69.97$ {\scriptsize $(69.91 \pm 0.37)$} &
     $75.21$ {\scriptsize $(75.20 \pm 0.41)$ ***} \\
    
    $\min\{\textrm{Swish}(x), \alpha \textrm{ELU}(\textrm{ReLU}(\beta x))\}$ & 
     $72.44$ {\scriptsize $(72.39 \pm 0.29)$ ***} &
     $69.90$ {\scriptsize $(69.82 \pm 0.40)$} &
     $75.20$ {\scriptsize $(75.27 \pm 0.38)$ ***} \\
    
    $\log(\sigma(x))$ & 
     $72.38$ {\scriptsize $(72.33 \pm 0.32)$ ***} &
     $69.49$ {\scriptsize $(69.58 \pm 0.35)$} &
     \boldsymbol{$75.45$} {\scriptsize $(75.53 \pm 0.37)$ ***} \\
    \midrule
    
    \textbf{Fixed Baseline Functions}\\
    $\textrm{ReLU}$ &
    $71.44$ {\scriptsize $(71.46 \pm 0.50)$} &
    $69.78$ {\scriptsize $(69.64 \pm 0.65)$} &
    $74.43$ {\scriptsize $(74.39 \pm 0.44)$} \\

    $\textrm{ELiSH}$ & 
     $01.00$ {\scriptsize $(01.00 \pm 0.00)$} &
    $01.00$ {\scriptsize $(01.00 \pm 0.00)$} &
    $75.16$ {\scriptsize $(75.20 \pm 0.31)$ ***} \\
    
    $\textrm{ELU}$ & 
     $72.41$ {\scriptsize $(72.30 \pm 0.32)$ ***} &
    $69.59$ {\scriptsize $(69.67 \pm 0.46)$} &
    $74.86$ {\scriptsize $(74.95 \pm 0.30)$ **} \\
    
    $\textrm{GELU}$ & 
     $72.00$ {\scriptsize $(71.95 \pm 0.35)$ *} &
    $70.16$ {\scriptsize $(70.19 \pm 0.40)$ *} &
    $74.84$ {\scriptsize $(74.86 \pm 0.33)$ **} \\
    
    $\textrm{HardSigmoid}$ & 
     $55.55$ {\scriptsize $(54.99 \pm 1.00)$} &
    $33.31$ {\scriptsize $(32.55 \pm 4.06)$} &
    $65.03$ {\scriptsize $(64.90 \pm 0.69)$} \\
    
    $\textrm{Leaky ReLU}$ & 
     $71.76$ {\scriptsize $(71.73 \pm 0.33)$} &
    $69.77$ {\scriptsize $(69.78 \pm 0.33)$} &
    $74.75$ {\scriptsize $(74.73 \pm 0.35)$ *} \\
    
    $\textrm{Mish}$ & 
     $72.02$ {\scriptsize $(71.95 \pm 0.41)$ *} &
    $70.03$ {\scriptsize $(69.88 \pm 0.54)$} &
    $75.33$ {\scriptsize $(75.32 \pm 0.29)$ ***} \\
    
    $\textrm{SELU}$ & 
     $70.55$ {\scriptsize $(70.53 \pm 0.42)$} &
    $68.51$ {\scriptsize $(68.52 \pm 0.29)$} &
    $73.86$ {\scriptsize $(73.79 \pm 0.36)$} \\
    
    $\textrm{sigmoid}$ & 
     $56.45$ {\scriptsize $(56.10 \pm 0.98)$} &
    $37.07$ {\scriptsize $(36.47 \pm 3.32)$} &
    $66.72$ {\scriptsize $(66.45 \pm 0.92)$} \\
    
    $\textrm{Softplus}$ & 
     $72.25$ {\scriptsize $(72.27 \pm 0.26)$ ***} &
    $69.71$ {\scriptsize $(69.71 \pm 0.36)$} &
    \boldsymbol{$75.47$} {\scriptsize $(75.46 \pm 0.52)$ ***} \\
    
    $\textrm{Softsign}$ & 
     $56.72$ {\scriptsize $(56.30 \pm 2.16)$} &
    $58.33$ {\scriptsize $(58.38 \pm 0.96)$} &
    $69.31$ {\scriptsize $(69.33 \pm 0.39)$} \\
    
    $\textrm{Swish}$ & 
     $72.27$ {\scriptsize $(72.26 \pm 0.28)$ ***} &
    $69.60$ {\scriptsize $(69.68 \pm 0.38)$} &
    $75.17$ {\scriptsize $(75.08 \pm 0.36)$ ***} \\
    
    $\textrm{tanh}$ & 
     $56.29$ {\scriptsize $(56.52 \pm 1.53)$} &
    $63.89$ {\scriptsize $(63.88 \pm 0.38)$} &
    $70.53$ {\scriptsize $(70.44 \pm 0.40)$} \\
    \midrule
    
    \textbf{Parametric Baseline Functions}\\
    % Moved to appendix
    % $\alpha \textrm{ReLU}(\beta x)$ & 
    % $72.01$ {\scriptsize $(71.96 \pm 0.31)$ **} &
    % $68.91$ {\scriptsize $(68.93 \pm 0.22)$} &
    % $73.60$ {\scriptsize $(73.52 \pm 0.37)$} \\
    
    % $\alpha \textrm{ELiSH}(\beta x)$ & 
    % $01.00$ {\scriptsize $(01.00 \pm 0.00)$}&
    % $01.00$ {\scriptsize $(01.00 \pm 0.00)$}&
    % $73.95$ {\scriptsize $(73.94 \pm 0.33)$}\\
    
    % $\alpha \textrm{ELU}(\beta x)$ & 
    % $71.96$ {\scriptsize $(71.98 \pm 0.24)$ **} &
    % $68.91$ {\scriptsize $(69.06 \pm 0.37)$} &
    % $74.03$ {\scriptsize $(73.97 \pm 0.45)$} \\
    
    % $\alpha \textrm{GELU}(\beta x)$ & 
    % $71.86$ {\scriptsize $(71.96 \pm 0.34)$ **} &
    % $69.35$ {\scriptsize $(69.39 \pm 0.35)$} & 
    % $73.77$ {\scriptsize $(73.83 \pm 0.24)$} \\
    
    % $\alpha \textrm{HardSigmoid}(\beta x)$ & 
    % $66.74$ {\scriptsize $(66.70 \pm 0.64)$} &
    % $33.47$ {\scriptsize $(34.33 \pm 6.53)$} &
    % $65.09$ {\scriptsize $(65.10 \pm 0.40)$} \\ 
    
    % $\alpha \textrm{Leaky ReLU}(\beta x)$ & 
    % $71.70$ {\scriptsize $(71.74 \pm 0.39)$} &
    % $69.18$ {\scriptsize $(69.11 \pm 0.47)$} &
    % $73.53$ {\scriptsize $(73.44 \pm 0.29)$} \\ 
    
    % $\alpha \textrm{Mish}(\beta x)$ & 
    % $72.02$ {\scriptsize $(72.11 \pm 0.31)$ **} &
    % $69.66$ {\scriptsize $(69.51 \pm 0.67)$} &
    % $73.72$ {\scriptsize $(73.72 \pm 0.32)$} \\
    
    % $\alpha \textrm{SELU}(\beta x)$ & 
    % $71.04$ {\scriptsize $(71.07 \pm 0.33)$} &
    % $68.06$ {\scriptsize $(68.05 \pm 0.39)$} &
    % $73.44$ {\scriptsize $(73.37 \pm 0.38)$} \\
    
    % $\alpha \textrm{sigmoid}(\beta x)$ & 
    % $67.16$ {\scriptsize $(66.98 \pm 0.66)$} &      
    % $43.72$ {\scriptsize $(44.40 \pm 2.62)$} &
    % $66.80$ {\scriptsize $(66.98 \pm 0.85)$} \\ 
    
    % $\alpha \textrm{Softplus}(\beta x)$ & 
    % $71.82$ {\scriptsize $(71.73 \pm 0.31)$} &
    % $68.84$ {\scriptsize $(68.84 \pm 0.30)$} &
    % $73.92$ {\scriptsize $(73.95 \pm 0.37)$} \\ 
    
    % $\alpha \textrm{Softsign}(\beta x)$ & 
    % $62.19$ {\scriptsize $(62.12 \pm 0.83)$} &
    % $01.00$ {\scriptsize $(9.18 \pm 13.75)$} &
    % $68.91$ {\scriptsize $(68.87 \pm 0.38)$} \\ 
    
    % $\alpha \textrm{Swish}(\beta x)$ & 
    % $72.36$ {\scriptsize $(72.26 \pm 0.29)$ ***} &
    % $69.25$ {\scriptsize $(69.25 \pm 0.28)$} &
    % $73.97$ {\scriptsize $(73.93 \pm 0.22)$} \\ 
    
    % $\alpha \textrm{tanh}(\beta x)$ & 
    % $63.72$ {\scriptsize $(63.55 \pm 0.56)$} &
    % $01.00$ {\scriptsize $(02.92 \pm 6.07)$} &
    % $69.61$ {\scriptsize $(69.55 \pm 0.62)$} \\ 
    
    $\textrm{PReLU}$ &
    $72.25$ {\scriptsize $(72.23 \pm 0.37)$ ***} &
    $69.67$ {\scriptsize $(69.77 \pm 0.40)$} &
    $74.99$ {\scriptsize $(75.10 \pm 0.53)$ **} \\

    $\textrm{PSwish} = x \cdot \sigma(\beta x)$ & 
    $72.46$ {\scriptsize $(72.40 \pm 0.31)$ ***} &
    $70.19$ {\scriptsize $(70.16 \pm 0.46)$ *} &
    \boldsymbol{$75.37$} {\scriptsize $(75.39 \pm 0.28)$ ***} \\
    \midrule
    
    \textbf{Learnable Baseline Functions}\\
    $\textrm{APL}$ &
    $72.91$ {\scriptsize $(72.88 \pm 0.32)$ ***} &
    \boldsymbol{$70.88$} {\scriptsize $(70.81 \pm 0.20)$ ***} &
    $74.94$ {\scriptsize $(75.02 \pm 0.28)$ ***} \\

    $\textrm{PAU}$ &
    $45.85$ {\scriptsize $(41.46 \pm 22.66)$} &
    $01.00$ {\scriptsize $(01.00 \pm 0.00)$} &
    $01.00$ {\scriptsize $(02.38 \pm 4.36)$} \\
    
    $\textrm{SPLASH}$ &
    $72.25$ {\scriptsize $(72.16 \pm 0.81)$ *} &
    $01.00$ {\scriptsize $(01.00 \pm 0.00)$} &
    $73.54$ {\scriptsize $(73.45 \pm 0.43)$} \\
    
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    % \vspace{-2em}
    \label{tab:results}
\end{table*}

==> figures/scatter_hist.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/scatter_hist.pdf}
    \caption{Fitness (validation accuracy) and compute cost (runtime in hours) among all activation functions considered in two independent PANGAEA processes.  Each point represents a unique activation function.  The distribution of fitness and compute cost are shown in histograms on the top and right, respectively.  Both PANGAEA processes reliably discover many novel activation functions that outperform ReLU.}
    \label{fig:scatter_hist}
\end{figure}
